The flip-graph of the 4-dimensional cube is connected

Flip-graph connectedness is established here for the vertex set of the 4-dimensional cube. It is found as a consequence that this vertex set has 92 487 256 triangulations, partitioned into 247 451 symmetry classes.

==> Proposition3/bash/enumerateLa <==
#!/bin/bash
# This bash script enumerates set L_a(S) where S is a subset
# of {0,1}^4/a so that kappa(a)\{a} is a subset of S. See the
# manuscript entitled: The flip-graph of the 4-dimensional
# cube is connected (by L. Pournin) for comprehensive
# explanations regarding all the notations, and the problem
# at hand.

# The following part of the code is dedicated to show the usage
# of the script when the option -h is specified.
usage()
{
cat << EOF
This script enumerates set L_a(S) for some subset S of {0,1}^4/a
that contains at least points b/a, c/a, e/a, and i/a. It needs
TOPCOM to be installed. Download TOPCOM from:

http://www.rambau.wm.uni-bayreuth.de/TOPCOM/

usage: $0 -a -p [b-o]

OPTIONS:
  -h   Shows this message
  -a   Checks all the triangulations of the provided points
       regardless of symetries (by default, finds symetries)
  -p   List of the vertices of the 4-dimensional cube [b-p]
       the points of S are the images of under the homogeneous
       contraction at point a 

EXAMPLES:
  $0 -a -p bcdefgi will check all the triangulations of
  the point configuration made up of points b/a,c/a,d/a,e/a,
  f/a,g/a, and i/a
EOF
}

# Reads the command line options. Flag testall is 0 when the
# calculation is restricted to the triangulations of S up to 
# symmetries. Each character of the  string pointconfiguration
# is one of the points of S.
testall=0
pointsconfiguration=""
while getopts “hap:” option
do 
  case $option in
    h)
      usage
      exit 1
      ;;
    a)
      testall=1
      ;;
    p)
      pointsconfiguration=$OPTARG
      ;;
    ?)
      usage
      exit
      ;;
  esac
done

# If the point configuration was not specified, displays the
# usage and exits.
if [[ -z $pointsconfiguration ]]
then
  usage
  exit 1
fi

start_time=`date +%s`

# An input for TOPCOM is now built from the string pointsconfiguration.
# This input contains the vector of coordinates of each point of S and
# will be stored in the string input_TOPCOM, that begins with the 
# character [.
input_TOPCOM="["

# The integer nbpoints will count the number of points provided by the
# user (that is, the number of characters in string pointsconfiguration).
nbpoints=0

# The string lst, here first initialized to an empty string be obtained
# from string pointsconfiguration by inserting space after each point.
# This string will be needed in order to compute the symmetries of the
# set S.
lst=""

# The string pointstogo initially contains all the points of S specified
# by the user with the option -p. These points are removed one by one
# from pointstogo as they are being handled. 
pointstogo=$pointsconfiguration

# The expression ${#pointstogo} is the length of string pointstogo. As
# a consequence, the following while loop exits when all the points
# have been removed from this string.
while [ ${#pointstogo} -gt 0 ]
do
  input_TOPCOM=$input_TOPCOM"\n"

  # Stores the first character of string pointstogo in string pt.
  pt=${pointstogo:0:1}
  
  # Removes the first character from the string pointstogo.
  pointstogo=${pointstogo:1:$[${#pointstogo}-1]}
  
  # Writes the coordinates of the image under the homogeneous contraction
  # at point a (note that, hereafter, x/a is also referred to as "x" when
  # no confusion is possible) of the point stored in string pt into the
  # string input_TOPCOM. These coordinates are chosen as follows: b is the
  # origin of R^3; c, e, and i are placed on the three axes at a multiple
  # of each basis vector (the multiplicative coefficient is 12 to allow
  # for easy divisions). The other coordinates are obtained from these
  # four points according to figure 1 in the manuscript. The fourth
  # coordinate is the homogeneization coordinate required by TOPCOM.
  case $pt in
    b)
      input_TOPCOM=$input_TOPCOM"[0,0,0,1],"
      ;;
    c)
      input_TOPCOM=$input_TOPCOM"[12,0,0,1],"
      ;;
    d)
      input_TOPCOM=$input_TOPCOM"[6,0,0,1],"
      ;;
    e)
      input_TOPCOM=$input_TOPCOM"[0,12,0,1],"
      ;;
    f)
      input_TOPCOM=$input_TOPCOM"[0,6,0,1],"
      ;;
    g)
      input_TOPCOM=$input_TOPCOM"[6,6,0,1],"
      ;;
    h)
      input_TOPCOM=$input_TOPCOM"[4,4,0,1],"
      ;;
    i)
      input_TOPCOM=$input_TOPCOM"[0,0,12,1],"
      ;;
    j)
      input_TOPCOM=$input_TOPCOM"[0,0,6,1],"
      ;;
    k)
      input_TOPCOM=$input_TOPCOM"[6,0,6,1],"
      ;;
    l)
      input_TOPCOM=$input_TOPCOM"[4,0,4,1],"
      ;;
    m)
      input_TOPCOM=$input_TOPCOM"[0,6,6,1],"
      ;;
    n)
      input_TOPCOM=$input_TOPCOM"[0,4,4,1],"
      ;;
    o)
      input_TOPCOM=$input_TOPCOM"[4,4,4,1],"
      ;;
    p)
      input_TOPCOM=$input_TOPCOM"[3,3,3,1],"
      ;;
    ?)
      echo "unknown vertex $pt: vertices should be letters from a to p"
      exit 1
      ;;
  esac
  
  # Table vertex records the labels [b-p] of the points in the order
  # in th order they have been written in the string input_TOPCOM. For
  # example, if pointsconfiguration is the string bcei. then table
  # vertex will be so that vertex[0]=b/a, vertex[1]=c/a, vertex[2]=e/a,
  # and vertex[3]=i/a. This is important because TOPCOM labels the
  # vertices according to their order in the input (that is, here, in
  # the string input_TOPCOM. In order to translate the output of TOPCOM,
  # table vertex will therefore be needed.
  vertex[$nbpoints]=$pt

  lst="$lst$pt "
  nbpoints=$[$nbpoints+1]
done

input_TOPCOM=$input_TOPCOM"\n]\n\n[\n"

# Now the symmetries of point configuration S are computed by checking
# invariance of string lst with respect to character permutations that
# correspond to possible symmetries of point configuration S.

sym[0]=$(echo $lst | sed "s/o/q/g" | sed "s/n/o/g" | sed "s/h/n/g" | sed "s/q/h/g" | sed "s/m/q/g" | sed "s/f/m/g" | sed "s/g/f/g" | sed "s/q/g/g" | sed "s/i/q/g" | sed "s/b/i/g" | sed "s/c/b/g" | sed "s/q/c/g" | sed "s/k/q/g" | sed "s/j/k/g" | sed "s/d/j/g" | sed "s/q/d/g")
sym[1]=$(echo $lst | sed "s/o/q/g" | sed "s/n/o/g" | sed "s/l/n/g" | sed "s/q/l/g" | sed "s/g/q/g" | sed "s/f/g/g" | sed "s/d/f/g" | sed "s/q/d/g" | sed "s/m/q/g" | sed "s/j/m/g" | sed "s/k/j/g" | sed "s/q/k/g" | sed "s/e/q/g" | sed "s/b/e/g" | sed "s/c/b/g" | sed "s/q/c/g")
sym[2]=$(echo $lst | sed "s/e/q/g" | sed "s/c/e/g" | sed "s/i/c/g" | sed "s/q/i/g" | sed "s/m/q/g" | sed "s/g/m/g" | sed "s/k/g/g" | sed "s/q/k/g" | sed "s/n/q/g" | sed "s/h/n/g" | sed "s/l/h/g" | sed "s/q/l/g" | sed "s/j/q/g" | sed "s/f/j/g" | sed "s/d/f/g" | sed "s/q/d/g")
sym[3]=$(echo $lst | sed "s/e/q/g" | sed "s/b/e/g" | sed "s/i/b/g" | sed "s/q/i/g" | sed "s/m/q/g" | sed "s/f/m/g" | sed "s/j/f/g" | sed "s/q/j/g" | sed "s/o/q/g" | sed "s/h/o/g" | sed "s/l/h/g" | sed "s/q/l/g" | sed "s/k/q/g" | sed "s/g/k/g" | sed "s/d/g/g" | sed "s/q/d/g")
sym[4]=$(echo $lst | sed "s/d/q/g" | sed "s/j/d/g" | sed "s/q/j/g" | sed "s/h/q/g" | sed "s/n/h/g" | sed "s/q/n/g" | sed "s/g/q/g" | sed "s/m/g/g" | sed "s/q/m/g" | sed "s/c/q/g" | sed "s/i/c/g" | sed "s/q/i/g")
sym[5]=$(echo $lst | sed "s/b/q/g" | sed "s/c/b/g" | sed "s/q/c/g" | sed "s/f/q/g" | sed "s/g/f/g" | sed "s/q/g/g" | sed "s/n/q/g" | sed "s/o/n/g" | sed "s/q/o/g" | sed "s/j/q/g" | sed "s/k/j/g" | sed "s/q/k/g")
sym[6]=$(echo $lst | sed "s/b/q/g" | sed "s/i/b/g" | sed "s/q/i/g" | sed "s/f/q/g" | sed "s/m/f/g" | sed "s/q/m/g" | sed "s/h/q/g" | sed "s/o/h/g" | sed "s/q/o/g" | sed "s/d/q/g" | sed "s/k/d/g" | sed "s/q/k/g")
sym[7]=$(echo $lst | sed "s/c/q/g" | sed "s/e/c/g" | sed "s/q/e/g" | sed "s/d/q/g" | sed "s/f/d/g" | sed "s/q/f/g" | sed "s/k/q/g" | sed "s/m/k/g" | sed "s/q/m/g" | sed "s/l/q/g" | sed "s/n/l/g" | sed "s/q/n/g")
sym[8]=$(echo $lst | sed "s/b/q/g" | sed "s/e/b/g" | sed "s/q/e/g" | sed "s/j/q/g" | sed "s/m/j/g" | sed "s/q/m/g" | sed "s/d/q/g" | sed "s/g/d/g" | sed "s/q/g/g" | sed "s/l/q/g" | sed "s/o/l/g" | sed "s/q/o/g")
sym[9]=$(echo $lst | sed "s/e/q/g" | sed "s/i/e/g" | sed "s/q/i/g" | sed "s/g/q/g" | sed "s/k/g/g" | sed "s/q/k/g" | sed "s/f/q/g" | sed "s/j/f/g" | sed "s/q/j/g" | sed "s/h/q/g" | sed "s/l/h/g" | sed "s/q/l/g")

# The symmetries found are stored in format used by TOPCOM in the string symlist.

symlist=""
for i in 0 1 2 3 4 5 6 7 8 9
do
  if [ "$(echo ${sym[$i]} | tr " " "\n" | sort | tr "\n" " ")" = "$lst" ]
  then
    symlist=$symlist"[$(echo ${sym[$i]} | sed "s/ /,/g")],"
  fi
done

# Here, the points in string symlist are still labeled with letters. Before calling TOPCOM, these
# labels have to be changed into integers according to their order kept in table vertex.
i=$nbpoints
while [ $i -gt 0 ]
do
  i=$[$i-1]
  symlist=$(echo $symlist | sed "s/"${vertex[$i]}"/"$i"/g")
done

if [ "$symlist" != "" ]
then
  input_TOPCOM=$input_TOPCOM${symlist:0:$[${#symlist}-1]}"\n]"
fi

# TOPCOM is now called in order to compute the triangulations of set S. If the option -a was
# specified, a complete enumeration is done. Otherwise, only the triangulations that are connected
# by flips to a regular triangulation are computed. Observe that the flip graphs of S_1, S_2, and
# S_3 are connected (this can be checked with TOPCOM). Therefore, when the -a option is not
# specified, TOPCOM enumerates all the triangulations of these point configurations anyway. In
# addition, when the option -a is not specified, then TOPCOM uses the symmetries provided and
# only returns triangulations that are not isometric to one another. The resulting list of
# triangulations is stored in the string tmp.
 
echo -n "calling TOPCOM to compute triangulations of point configuration $pointsconfiguration/a... "
if [ $testall -eq 1 ]
then
  tmp=$(echo -e $input_TOPCOM | points2chiro 2>&- | chiro2alltriangs 2>&-)
else
  tmp=$(echo -e $input_TOPCOM | points2chiro 2>&- | chiro2triangs 2>&- | sed "s/"T\[[0-9]*\]:=\[[0-9,]*:"//g" | sed "s/\];//g")
fi

# Replaces the integer labels returned by TOPCOM for the points of S in every triangulation of S
# by characters [b-p] according to array vertex. The triangulations are then stored into the array
# triangs. Each line in this array contains a string that defines one circuit of set S and its
# Radon partition. For example, the string {b,i},{j} represents circuit {b,i,j}/a whose Radon
# partition is {{b,i},{j}}/a. Integer nbtri counts the number of triangulations found.
nbtri=0
for i in $tmp
do
  tri=$i
  j=$nbpoints
  while [ $j -gt 0 ]
  do
    j=$[$j-1]
    tri=$(echo $tri | sed "s/$j/${vertex[$j]}/g")
  done
  triangs[$nbtri]=$tri
  nbtri=$[$nbtri+1]
done

echo $nbtri triangulations found.

# Calls TOPCOM to compute the circuits of point configuration S. The resulting circuits
# are stored in the string tmp.
echo "calling TOPCOM to compute circuits of point configuration $pointsconfiguration/a... "
tmp=$(echo -e $input_TOPCOM | points2chiro 2>&- | chiro2circuits 2>&-)

# Replaces the integer labels returned by TOPCOM for the points of S in every circuit of S
# by characters [b-p] according to array vertex. The replacement is made directly into
# string tmp.
i=$nbpoints
while [ $i -gt 0 ]
do
  i=$[$i-1]
  tmp=$(echo $tmp | sed "s/$i/${vertex[$i]}/g")
done

# Calls TOPCOM to compute the circuits of {0,1}^4/a. The resulting circuits
# are stored in the string tmp2. Observe here that the command cube is
# installed together with TOPCOM.
echo "calling TOPCOM to compute the circuits of the 4-dimensional cube..."
tmp2=$(cube 4 | points2chiro 2>&- | chiro2circuits 2>&- | sed "s/15/p/g" | sed "s/14/o/g" | sed "s/13/n/g" | sed "s/12/m/g" | sed "s/11/l/g" | sed "s/10/k/g" | sed "s/9/j/g" | sed "s/8/i/g" | sed "s/7/h/g" | sed "s/6/g/g" | sed "s/5/f/g" | sed "s/4/e/g" | sed "s/3/d/g" | sed "s/2/c/g" | sed "s/1/b/g" | sed "s/0/a/g")

# Finds the circuits of point configuration S that belong to Z(a)/a. These
# circuits are stored in the array circuits. Each entry in this array is a
# string that defines one circuit of {0,1}^4/a, its Radon partition, and
# the two sets epsilon_a^-(z)/a and epsilon_a^+(z)/a (see the manuscript
# for details on these notations). For example, the string {f,l},{d,e,j}
# represents circuit {d,e,f,j,l}/a, so that epsilon_a^-(z)/a={f,l}/a and
# epsilon_a^+(z)/a={d,e,j}/a. In addition, recall that for any such circuit
# z/a, epsilon_a^-(z)/a and epsilon_a^+(z)/a are the two elements of the
# Radon partition of z/a. As a consequence, the Radon partition of the
# circuit represented by this string is indeed {{f,l},{d,e,j}}/a.
echo -n "finding the circuits of point configuration $pointsconfiguration/a that belong to Z(a)/a... "

# Integer nbcir counts the number of circuits of S found in Z(a)/a
nbcir=0
for i in $tmp
do
  if [ $(echo $i | grep -c ":") -eq 0 ] && [ ${#i} -gt 2 ]
  then
    cir=${i:2:$[${#i}-4]}
    cir=$(echo $cir | sed "s/},{/"\ "/g")

    part=($cir)
    f1=$(echo -e $tmp2 | grep -c "{a,${part[0]}},{${part[1]}}")
    f2=$(echo -e $tmp2 | grep -c "{a,${part[1]}},{${part[0]}}")

    if [ $f1 -ne 0 ] || [ $f2 -ne 0 ]
    then
      if [ $f1 -eq 0 ]
      then
        circuits[$nbcir]="{{${part[1]}},{${part[0]}}}"
      else
        circuits[$nbcir]="{{${part[0]}},{${part[1]}}}"
      fi
      nbcir=$[$nbcir+1]
    fi
  fi
done

echo $nbcir circuit found.

# For all the circuits z stored in array circuits, computes the triangulation
# of z/a that contains epsilon_a^-(z)/a, referred to as tau^- hereafter. See
# the manuscript for more details. These triangulations are stored in array
# tau. The i-th element of this array is a string that gives the triangulation
# tau^- of the circuit z stored in the i-th line of array circuits. For
# example, if line 3 of tau is string "flej fldj flde" then the triangulation
# tau^- of the circuit z stored in line 3 of array circuits is the
# triangulation that contains {f,l,e,j}/a, {f,l,d,j}/a, and {f,l,d,e}/a as its
# three elements of maximal dimension. Observe that the vertices of each
# simplex in every triangulation are sorted in ascending alphabetical order.
echo "computing the triangulations tau^- for every z in Z(a)/a... "

i=0
while [ $i -lt $nbcir ]
do
  tmp=""
  cir=${circuits[$i]}
  Radon_partition=${cir:2:$[${#cir}-4]}
  Radon_partition=$(echo $Radon_partition | sed "s/},{/"\ "/g")

  part=($Radon_partition)

  for pt in $(echo ${part[1]} | sed "s/,/"\ "/g")
  do
    simplex=$(echo $Radon_partition | sed "s/"\ "/,/g" | sed "s/,$pt//g" | sed "s/$pt,//g" | sed "s/$pt//g")
    tmp="$tmp$(echo $simplex | tr "," "\n" | sort | tr -d "\n") "
  done
  tau[$i]=$tmp
  i=$[$i+1]
done

# Finds all the triangulations in La(S) and store them into the cell array
# La. This is done following  algorithm 1 found in the manuscript. Some
# variations from algorithm 1 have will be found whose only incidence is
# on the efficiency of the calculation. They will be mentioned below.
sizeLa=0

# Index i points to the i-th triangulation of S, found as element i of array
# triangs.
i=0
while [ $i -lt $nbtri ]
do
  # String tri stores the i-th triangulation of S.
  tri=${triangs[$i]}
  tri=${tri:2:$[${#tri}-4]}
  tri=$(echo $tri | sed "s/},{/"\ "/g")

  # Now the circuits in array circuits will be considered one by one. The
  # flag f1 will be equal to 1 if the circuit considered prevents the
  # triangulation tri to be in La, and to 0 otherwise. This flag is
  # initially set to 0, and the search will finish as soon as a circuit is
  # found that prevents triangulation tri to be in La. The first
  # difference with the algorithm given in the manuscript is that only one
  # flag is used here (whereas two flags f1 and f2 are used in the
  # manuscript for readability).
  f1=0

  # Index j points to the j-th circuit, found in row j of cell array
  # circuits. It is initially equal to zero and will be incremented in the
  # while loop below.
  j=0

  # Here, the condition in the while loop will cause an exit either if all
  # the circuits have been tested or if a circuit is found that prevents
  # triangulation tri to be in La (this occurs when at the end of the while
  # loop flag f1 is equal to 1).
  while [ $j -lt $nbcir ] && [ $f1 -eq 0 ]
  do
    # string cir stores circuit j. 
    cir=${circuits[$j]}

    # A preliminary check is performed to verify that all the vertices of
    # circuit cir are vertices of triangulation tri. Otherwise, the
    # circuit does not prevent the triangulation to be in La (because of
    # theorem 2 in the manuscript). The flag circuit_is_ok is initially
    # set to 1 and will be changed to 0 whenever a point of circuit cir
    # is not a vertex of triangulation tri. 
    circuit_is_ok=1

    for k in $(echo $cir | sed "s/}//g" | sed "s/{//g" | sed "s/,/"\ "/g")
    do
      if [ $(echo $tri | grep -c $k) -eq 0 ]
      then
        circuit_is_ok=0
        break
      fi
    done

    if [ $circuit_is_ok -eq 1 ]
    then
      # First, array tmptau is initialized. Its elements are the maximal 
      # simplices of triangulation tau^- of circuit cir
      tmptau=(${tau[$j]})

      # The first simplex in the triangulation tau^- of cir is stored in
      # the string simplex.
      simplex=${tmptau[0]}

      # Now, it will be checked whether the simplex stored in the string
      # simplex is an element of the triangulation tri (equivalently, that
      # all the characters of string simplex are found in a same tetrahedron
      # in string tri). If simplex is an element of tri, its link in tri
      # is computed simulmtaneously and stored in the string link1.
      link1=""

      # The following for loop will consider one by one all the tetrahadra
      # of triangulation tri, stored in the string tetra. 
      for tetra in $tri
      do
        # This instruction removes every character of the string simplex from
        # the string tetra and stores the result in the string tmplink.
        tmplink=$(echo $tetra | sed "s/['$simplex',]//g")

        # If the number of characters removed from string tetra is equal
        # to the number of characters in the string simplex then this simplex
        # is a subset of tetrahadron tetra, and tmplink is an element of its
        # link in triangulation tri. In this case tmplink is concatenated with
        # link1 and flag f1 is set to 1. This flag can still be changed to 0
        # in the while loop below if another maximal simplex in triangulation
        # tau^- of cir is not found in the triangulation, or if its link in
        # triangulation tri is not equal to link1.
        if [ $[${#tmplink}+${#simplex}] -eq 4 ]
        then
          link1="$link1$tmplink "
          f1=1
        fi
      done

      # The simplices in link1 are sorted in ascending lexicographic order
      link1=$(echo $link1 | tr " " "\n" | sort | tr "\n" " ")

      # The remaining simplices in tmptau are now checked in a while loop.
      # Observe that this while loop is only executed if f1=1 (that is, if
      # the first simplex of tau^- of cir was found in triangulation tri).
      # For each of these simplices, stored in the string simplex, it is
      # checked that this simplex is found in triangulation tri and that
      # its link in tri is equal to link1. If one of these two conditions
      # are not satisfied, then f1 will be set to 0 and the loop will
      # terminate. The loop alternatively terminates when all the
      # simplices in triangulation tau^- of cir have been found in
      # triangulation tri, and admit link1 as their link in tri. In this
      # case, circuit cir prevents triangulation tri to be in La.	  

      # Integer k is the index of the simplex to be checked in array tmptau
      k=1
      while [ $k -lt ${#tmptau[@]} ] && [ $f1 -eq 1 ]
      do
        simplex=${tmptau[$k]}

        # String link2 will store the link of simplex is this simplex is
        # found in triangulation tri. It will be later compared to link1.
        link2=""

        # The following for loop will consider one by one all the tetrahadra
        # of triangulation tri. These tetrahedra will be stored in the string
        # tetra. Flag f1 is reset to 0 and will be set to 1 in the for loop
        # if simplex is found as a subset of an element of triangulation tri.
        f1=0
        for tetra in $tri
        do
          # This instruction removes every character of the string simplex from
          # the string tetra and stores the result in the string tmplink.
          tmplink=$(echo $tetra | sed "s/['$simplex',]//g")

          # Again, if the number of characters removed from string tetra is equal
          # to the number of characters in the string simplex then this simplex is
          # a subset of tetrahadron tetra, and tmplink is an element of its link
          # in triangulation tri. In this case tmplink is concatenated with link2.
          if [ $[${#tmplink}+${#simplex}] -eq 4 ]
          then
            link2="$link2$tmplink "
            f1=1
          fi
        done

         # The simplices in link2 are sorted in ascending lexicographic order        
        link2=$(echo $link2 | tr " " "\n" | sort | tr "\n" " ")

        if [ "$link1" != "$link2" ]
        then
          f1=0
        fi
        k=$[$k+1]
      done
    fi

    # If A circuit is found that prevents triangulation tri to be in La
    # then this circuit is stored in circuit_found to be displayed
    # later.
    if [ $f1 -eq 1 ]
    then
      circuit_found=$cir
    fi

    # Increases the index j of the circuit
    j=$[$j+1]
  done
  i=$[$i+1]

  # If f1=0 then no circuit was found that prevents triangulation tri to
  # be in La. So tri is stored in the last row of cell array La.
  if [ $f1 -eq 0 ]
  then
    echo -e "\\033[1;31m"$i over $nbtri: triangulation {$(echo $tri | sed "s/,//g" | sed "s/\ /,/g")}/a belongs to La\(S\)"\\033[1;0m"
    La[$sizeLa]=$tri
    sizeLa=$[$sizeLa+1]
  else
    echo -e "$i over $nbtri: triangulation {$(echo $tri | sed "s/,//g" | sed "s/\ /,/g")}/a is not in La(S) because of circuit {$(echo $circuit_found | sed "s/,//g" | sed "s/}{/","/g" | sed "s/}//g" | sed "s/{//g")}/a."
  fi
done
finish_time=`date +%s`
duration=$[$finish_time-$start_time]

# Finally displays set La and its size.
echo ""
if [ $sizeLa -eq 1 ]
then
  echo "Found the following unique triangulations in La({$(echo $lst | sed "s/\ /,/g")}/a):"
else
  echo "Found the following $sizeLa triangulations in La({$(echo $lst | sed "s/\ /,/g")}/a):"
fi
i=0
while [ $i -lt $sizeLa ]
do
  echo "$[$i+1]: pi_a({$(echo ${La[i]} | sed "s/,//g" | sed "s/\ /,/g")})"
  i=$[$i+1]
done
echo ""
echo "Elapsed time: $duration seconds"




